Diffuse Lyman-alpha Halos around ~300 Spectroscopically Confirmed Lyman-alpha Emitters at z ~ 5.7

We report the detection of diffuse Lyman-alpha halos (LAHs) around star-forming galaxies at $z \sim 5.7$ by stacking 310 spectroscopically confirmed Lyman-alpha (LAEs). The majority of the LAEs are identified from our spectroscopic survey of galaxies at $z>5.5$. They are all located in well-studied fields with deep narrowband and broadband imaging data. We combine the LAE sample and its subsamples in the narrowband NB816 (i.e., the Lyman-alpha band) and $z$ band (i.e., the continuum band). By comparing the stacked objects with their corresponding point spread functions, we clearly detect extended LAHs around these LAEs. We perform sophisticated simulations and analyses on statistical and systematic errors, and confirm that the detected halos are not caused by errors. The scale lengths of the LAHs, when described by a double-component model, range from 1.2 to 5.3 kpc with a typical value of $\sim$2 kpc. The LAH sizes from our sample are in agreement with those of individual LAEs at the similar redshift measured by VLT/MUSE, but are relatively smaller than those of photometrically selected LAEs in previous studies. We also find that LAEs with higher Lyman-alpha luminosities, higher UV continuum luminosities or smaller Lyman-alpha equivalent widths tend to have larger LAH sizes. Our results are consistent with a scenario that LAHs originate from the scattered light of the central galaxies by H I gas in the circumgalactic medium.

==> compileTex <==
#!/bin/bash
set -e
file=Paper
if [[ main.tex -nt backup.tex ]]; then
    if [[ -f backup.tex ]]; then
        echo "update last.tex"
        cp backup.tex last.tex
    fi
    echo "update backup.tex"
    cp ${file}.tex backup.tex
fi
# cat `find ../references/*.bib | grep -v "all\.bib"` > ../references/all.bib
#pdflatex ${file} && bibtex ${file} && pdflatex ${file}
pdflatex ${file}  && bibtex ${file} && pdflatex ${file} && pdflatex ${file}
#open ${file}.pdf

